Checker Bug Detection and Repair in Deep Learning Libraries

Checker bugs in Deep Learning (DL) libraries are critical yet not well-explored. These bugs are often concealed in the input validation and error-checking code of DL libraries and can lead to silent failures, incorrect results, or unexpected program behavior in DL applications. Despite their potential to significantly impact the reliability and performance of DL-enabled systems built with these libraries, checker bugs have received limited attention. We present the first comprehensive study of DL checker bugs in two widely-used DL libraries, i.e., TensorFlow and PyTorch. Initially, we automatically collected a dataset of 2,418 commits from TensorFlow and PyTorch repositories on GitHub from Sept. 2016 to Dec. 2023 using specific keywords related to checker bugs. Through manual inspection, we identified 527 DL checker bugs. Subsequently, we analyzed these bugs from three perspectives, i.e., root causes, symptoms, and fixing patterns. Using the knowledge gained via root cause analysis of checker bugs, we further propose TensorGuard, a proof-of-concept RAG-based LLM-based tool to detect and fix checker bugs in DL libraries via prompt engineering a series of ChatGPT prompts. We evaluated TensorGuard's performance on a test dataset that includes 92 buggy and 135 clean checker-related changes in TensorFlow and PyTorch from January 2024 to July 2024. Our results demonstrate that TensorGuard has high average recall (94.51\%) using Chain of Thought prompting, a balanced performance between precision and recall using Zero-Shot prompting and Few-Shot prompting strategies. In terms of patch generation, TensorGuard achieves an accuracy of 11.1\%, which outperforms the state-of-the-art bug repair baseline by 2\%. We have also applied TensorGuard on the latest six months' checker-related changes (493 changes) of the JAX library from Google, which resulted in the detection of 64 new checker bugs.

==> section/background.tex <==
\section{Background and Related Work}
\label{sec:background}
\gias{background subsections can be removed if we explain in the introduction the checker bugs and the limitations of current techniques to detect and fixing of checker bugs}
\begin{comment}
\subsection{Significance of DL Libraries}
Much like traditional software, ML libraries are susceptible to various security bugs. This bugs arise because ML libraries share similar attack styles and deployment patterns at higher levels of granularity. However, when we fine the level of granularity, ML libraries tend to be more complex than traditional software in terms of design elements, as ML often involves complex mathematical models and algorithms~\cite{harzevili2023characterizing, thung2012empirical, islam2019comprehensive, jia2021symptoms}.
Generally, an AI applications have three elements, including data, algorithm, and hardware, that make it unique compared to traditional software.

\textbf{Data}: AI applications rely significantly on both the quantity and quality of data utilized during their training and inference processes. Concerning quantity, the sheer scale of data employed in AI applications is notably extensive compared to traditional software. Regarding quality, a substantial amount of data pre-processing, cleaning, and normalization is essential, aspects not typically addressed in traditional software.

\textbf{Algorithm}: AI applications often developed do perform sophisticated downstream tasks such as image classification \cite{algan2021image, mahdisoltani2018fine}, pattern recognition \cite{lv2022semi}, autonomous driving \cite{simhambhatla2019self, ramos2017detecting, kulkarni2018traffic}, and natural language processing \cite{minaee2017automatic, athreya2021template, roy2021deep}. To perform such tasks, AI applications leverage the benefits of ML APIs provided within ML libraries. These ML APIs are access point to sophisticated algorithm implementation in the backend of ML libraries. For example, one of the renowned tasks in image classification is done via pooling layer APIs\footnote{https://pytorch.org/docs/stable/nn.html\#pooling-layers}. The motivation for the pooling operation is to diminish the size of the feature map in the input, aiming to reduce the volume of training parameters. This reduction contributes to faster training times in machine learning models. 

\textbf{Hardware}: Indeed, AI applications generally have the capability to run on various devices, enabling high-performance computing. This flexibility is facilitated by DL libraries that are purposefully crafted to harness the capabilities of modern hardware, such as GPUs and specialized processors. This optimization across diverse hardware platforms contributes to enhanced performance in AI computations. Traditional software, on the other hand, is generally optimized for general-purpose CPUs. 

The discrepancies in design of AI applications served as a catalyst for initiating this thesis, aiming to comprehensively understand checker/validation bugs and their root causes within the context of ML libraries.
\end{comment}

\song{let's focus on these two topics}
\subsection{Checker Bugs}
Checker/validation bugs can have serious consequences since checking/validating malicious or unwanted data is crucial for software systems to ensure their security and reliability~\cite{lu2019detecting, zhan2022errhunter}. More specifically, in the context of DL libraries, previous studies~\cite{harzevili2023characterizing, harzevili2023automatic} reveal that the majority of bugs in these libraries result from missing or improper checkers in their implementation.

\subsection{LLM for Bug Detection and Repair}
The emergence of Large Language Models has had a profound impact on the field of software engineering research~\cite{wei2024demystifying, hossain2024deep, deng2023large1, deng2023large2}. 

==> section/evaluation.tex <==
\section{Evaluation}

\jinqiu{It is not very clear from the writing whether the ``Instances" in Figure 1 and the evaluation dataset are separate datasets. They should be, right?}
\gias{We need a suite a research questions to report the effectiveness of TensorGuard over the baselines. Example RQs are follows: (RQ1) How accurate is TensorGuard to fix the checker bugs? (here you report the precision, recall, F1, accuracy of TensorGuard and compare those with the baselines. You also discuss the misclassification reasons of TensorGuard, i.e., if someone wanted to improve TensorGuard, how would they do that. (RQ2) How does each prompt template contribute to the overall performance of TensorGuard? (here you discuss how each prompt template performaed. One way to do that is apply TensorGuard with the template and see how it performs, i.e., one without a template and one with the template. This is similar to feature importance analyssi in ML models. (RQ3) Would the choice of differente prompt templates have offered better performance? (here you mutate each prompt template to a slightly different version and and see how the performance of TensorGuard changes. This can be useful to see if your template for a given prompt is the optimal one or not. (RQ4) Is TensorGuard effective equally to fix all types of checker bugs? (here you show the distribution of TensorGuard paerformance by the bug types and compare those again with the baselines). (RQ5) potential other research questions, such as the choice of zero vs few shot prompt templates}
In this paper, we designed two experiments to evaluate {\tool}'s performance. We chose to use GPT-3.5\_turbo, as it has proven effective in software engineering tasks, particularly code generation\cite{pornprasit2024fine}. Some code changes in our dataset have extensively deleted and added lines, which negatively impact {\tool}'s performance. Therefore, we limited the length of code changes to less than 10 lines of code (LOC). We set the 'temperature' parameter to its default value of 0.7. Due to the stochastic nature of LLMs, which can produce different outputs for the same input, we ran {\tool} 5 times on our input data. This approach ensured that our results were consistent and not just one-time occurrences. We ran {\tool} on 425 instances for the Zero-Shot setting and 384 instances for the Few-Shot setting. For the Few-Shot setting, we excluded cases from the \textit{Others} category within the root cause, as well as instances used for the Few-Shot prompting. In the Few-Shot setting, we implemented a type-specific approach for example selection. For each instance, we first extract the root cause of the checker bug, then use this root cause to query relevant samples from our rule set (as shown in Table~\ref{tab:nested_json_device_type}). For example, if the current instance relates to device type issues, {\tool} queries the rule set database using the key variable \textit{device type} to retrieve relevant examples. {\tool} then utilizes these retrieved instances as shot examples in its prompting process. This method ensures that the few-shot examples provided to the model are closely aligned with the specific type of checker bug being addressed, potentially improving the relevance and effectiveness of the model's responses.

\input{table_sources/rules}
\subsection{Results}


\begin{lstlisting}[numbers=left,numbersep=1pt,numberstyle=\small]
\end{lstlisting}




\jinqiu{Would be interesting to discuss the false positives of TensorGuard, in both bug detection and repair.}
\begin{lstlisting}[numbers=left,numbersep=1pt,numberstyle=\small]
# TensorGuard detects a missing check in the
code below:
void Compute(OpKernelContext* ctx) override {
    const Tensor& input = ctx->input(0);
    const Tensor& input_min_tensor = ctx-
    >input(1);
    const Tensor& input_max_tensor = ctx-
    >input(2);
    
# The checker is missed here. 

    int num_slices = 1;
    if (axis_ > -1) {
      num_slices = input.dim_size(axis_);
}
# Patch:
OP_REQUIRES(context, axis_ < input.dims(),
errors::InvalidArgument("Axis value must be
less than input dimension."));

# Fixing pattern
The common fixing pattern in the code change is
to use the `OP\_REQUIRES` macro to ensure a 
condition is met. In this case, the condition 
being checked is that the `axis\_` value is less
than the dimensions of the `input`. If the 
condition is not met, an `InvalidArgument` error
is raised.
\end{lstlisting}


\input{table_sources/tensorGuardPerfTable}

==> section/misc.tex <==
\section{Characteristics of DL Libraries Checker Bugs}
\label{sec:checkerChar}
\gias{here you can take my comments about characterization from the previous section. This section can have two subsections: Study Setup and Study Results. Under setup, you talk about data collection, keywords, etc. Under results, you discuss the taxonomy.}


\subsection{Taxonomy of Root Cause}


\subsubsection{Root Cause Elements}


\subsection{Taxonomy of Impact}

\subsection{Taxonomy of Fixing pattern}



==> section/related.tex <==
\section{Related Work}
\label{sec:related}

\subsection{LLM-based Program Repair}



\subsection{Checker Bugs in Traditional Software}

Tian and Ray~\cite{tian2017automatically}
is one of the prominent studies conducted to characterize and fix error handling bugs within traditional software, specifically, software systems developed in C language. They conducted a comprehensive study that led to the development of \textit{ErrDoc}, a tool that detects, characterizes, and autwomatically fixes different types sdof error-handling bugs.
e
Pakki et al~\cite{pakki2020exaggerated},

Wwang2018check    d  

wang2021amchex

yamaguchi2013chucky

% wu2021understanding, zhan2022errhunter, lu2019detecting, , min2015cross, situ2018vanguard, , , tan2008autoises, son2011rolecast, zhan2022errhunter}

==> table_sources/rules.tex <==
\begin{table}
\centering
\caption{Database of Type-Specific Examples for Few-Shot Setting.}
\small
\renewcommand{\arraystretch}{0.2}
\resizebox{1\columnwidth}{!}{%
\begin{tabular}{p{0.08\textwidth}p{0.53\textwidth}}
\hline
\textbf{Key} & \textbf{Value} \\
\hline
device type & \{ \\
& \hspace{1em}example1: \{ \\
& \hspace{2em}"Deleted lines": "-    if device\_type.lower() == \"cuda\":", \\
& \hspace{2em}"Added lines": "+    if device\_type and device\_type.lower() == \"cuda\":", \\
& \hspace{1em}\}, \\
& \hspace{1em}example2: \{ \\
& \hspace{2em}"Deleted lines": "-    if (indices.is\_cuda()) \{", \\
& \hspace{2em}"Added lines": "+    if (!indices.is\_cpu()) \{", \\
& \hspace{1em}\} \\
\} \\
...\\
\hline
\end{tabular}}
\label{tab:nested_json_device_type}
\end{table}
